What is being transferred in transfer learning?

One desired capability for machines is the ability to transfer their knowledge of one domain to another where data is (usually) scarce. Despite ample adaptation of transfer learning in various deep learning applications, we yet do not understand what enables a successful transfer and which part of the network is responsible for that. In this paper, we provide new tools and analyses to address these fundamental questions. Through a series of analyses on transferring to block-shuffled images, we separate the effect of feature reuse from learning low-level statistics of data and show that some benefit of transfer learning comes from the latter. We present that when training from pre-trained weights, the model stays in the same basin in the loss landscape and different instances of such model are similar in feature space and close in parameter space.

==> setting.tex <==
%\usepackage[papersize={17cm,24cm},margin=18mm,top=17mm,headsep=5mm]{geometry} 
%\usepackage[papersize={17cm,24cm},margin=13mm,top=17mm,headsep=5mm]{geometry} 
%\usepackage[utf8]{inputenc}
%\usepackage{xltxtra} % extras for XeLaTeX
%\usepackage{unicode-math}
%\usepackage{fullpage}
\usepackage{epsf}
\usepackage{fancyhdr}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{psfrag}
\usepackage[T1]{fontenc}
\usepackage{color}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{natbib}
%\bibliographystyle{chicago}
\usepackage{mathrsfs}
\usepackage{bm}
\usepackage{accents}
\usepackage{listings}
\usepackage[linesnumbered, ruled, vlined]{algorithm2e}
\usepackage[titletoc,toc,title]{appendix}
\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-6cm}
\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-4cm}
\addtolength{\textheight}{-1.1\headheight}
\addtolength{\textheight}{-\headsep}
\addtolength{\textheight}{-\footskip}
\setlength{\oddsidemargin}{0.5cm}
\setlength{\evensidemargin}{0.5cm}
%\usepackage{tikz}
%\usetikzlibrary{matrix,shapes,arrows,positioning,chains, calc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
  \settoheight{\widebarargheight}{\ensuremath{#1}}%
  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
    \hspace{0.3\widebarargdepth}%
    \addtolength{\widebarargheight}{0.3ex}%
    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
  {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
        \vskip 0.8ex
        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
        \dimen0=\hsize
        \advance\dimen0 by -3em
        \ifdim \wd\@tempboxa >\dimen0
                \hbox to \hsize{
                        \parindent 0em
                        \hfil 
                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                                {\bf #1.} #2
                                %%\unhbox\@tempboxa
                                } 
                        \hfil}
        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
        \fi
        }
\makeatother


\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage{times}
\usepackage{enumerate}
\usepackage{verbatim} % verbatim input
%\usepackage{titling} % customize title
\usepackage[titletoc,toc,title]{appendix}
\usepackage{csquotes} % context sensitive quotes
\usepackage{upquote} % allow correct quotes in verbatim
\usepackage[bottom]{footmisc} % put footnotes down at the bottom margin
%\usepackage[svgnames]{xcolor} % color pictures with SVG names
\usepackage{graphicx} % \includegraphics
%\usepackage[noend]{algpseudocode}
\usepackage[ruled]{algorithm2e}
\usepackage{thmtools}
\usepackage{thm-restate}

\usepackage[dvipsnames]{xcolor}
%\pagecolor[rgb]{0.2,0.2,0.2}
%\color[rgb]{1,1,1}
%\usepackage[dvipsnames]{xcolor}
%\usepackage{lmodern}
%\usepackage{authblk}

%\usepackage[colorlinks,linkcolor = Mahogany, urlcolor  = RedViolet, citecolor = RoyalBlue, anchorcolor = ForestGreen]{hyperref}
%\usepackage{cleveref}

%\usepackage{optidef}
%\usepackage{enumitem} % customize lists
%\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
%\setitemize{itemsep=2pt,topsep=4pt,parsep=0pt,partopsep=0pt}
%\usepackage{covington}  % for numbered linguistic examples
\usepackage{tikz}
\usetikzlibrary{matrix,shapes,arrows,positioning,chains, calc,backgrounds}
\usepackage[english]{babel} % multilinguality
%\usepackage{polyglossia} % newer alternative to babel
%\setdefaultlanguage{english} % see http://ctan.uib.no/macros/xetex/latex/polyglossia/polyglossia.pdf
%\setmainfont[Mapping=tex-text,Ligatures=TeX,Scale=1.0]{Linux Libertine O} 
%\setmonofont[Mapping=tex-text,Scale=MatchLowercase,LetterSpace=-2.0]{DejaVu Sans Mono}
%\setmathfont{Cambria Math}
%\setmathfont[math-style=upright,vargreek-shape=unicode]{Neo Euler}
%\setmathfont{Linux Libertine O}
\renewcommand{\baselinestretch}{1.04} % stretch distance between baselines
\frenchspacing % reduce space after sentence-final punctuation
\date{}
\setlength{\parindent}{1em}
\clubpenalty = 10000
\widowpenalty = 10000
\hfuzz = 2pt  % No warnings about margin overhangs less than this amount.
%\setlength{\belowcaptionskip}{-1.2em}
%Theorem Repeat solutions


%\usepackage[compact,noindentafter]{titlesec} % customize section headings
%\titlespacing{\section}{0pt}{2.7mm}{1.5mm} % left indent, space before, space after
%\titlespacing{\subsection}{0pt}{2mm}{1pt}
%\titlespacing{\subsubsection}{0pt}{1.2mm}{0.5pt}

%\newcommand\Volume{N} % BeLLS Volume number
%\newcommand\Voleditors{Jan Editor and Ed Janitor}
%\newcommand\Voltitle{The book title}
%\newcommand\VolISBN{N}
%\newcommand\VolDOI{N}

%\usepackage{natbib}
%\usepackage[style = alphabetic,citestyle=alphabetic,maxbibnames=99,backend=biber,natbib=true,backref=true]{biblatex}
%\addbibresource{bib.bib}
%\DefineBibliographyStrings{english}{%
 % backrefpage = {Cited on page},% originally "cited on page"
 % backrefpages = {Cited on pages},% originally "cited on pages"
%}
%\usepackage{fullname}
%\bibliographystyle{plain}
%\bibliographystyle{chicago} % chicago or spbasic or spmpsci or spphys
%\bibliographystyle{alphanat} % chicago  or spbasic or spmpsci or spphys
%\setlength{\bibhang}{-0.5em}
%\setlength{\bibsep}{0mm}
%\let\bibfont=\small
%\setcitestyle{numbers}

% footnote without number
% \newcommand\blfootnote[1]{
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{\hspace{-2.4em} #1}%
%   \addtocounter{footnote}{-1}
%   \endgroup
% }

% customize title
%\renewcommand{\maketitle}
%  {\bgroup\setlength{\parindent}{0pt}
%   \begin{flushleft}
%    \textbf{\LARGE{\ \\ \vspace{20mm}\strut\thetitle\strut}\vspace{2mm}}
%    
%    {\Large\theauthor}
%  \end{flushleft}\egroup\vspace{18mm}
%}

%% customize abstract
%\renewenvironment{abstract}
%  {\noindent\small %\quotation
%  {\noindent{\large\textbf\abstractname. }%\par\nobreak\smallskip
%  \thispagestyle{plain}
%  %\blfootnote{In: \emph{Volume title,} edited by Jan Editor and Ed Janitor. BeLLS Vol. N (2017), DOI N. Open Access under the terms of CC-BY-NC-4.0.}
%  }}
%  {}
%    
%% command in which to embed tabular material in numbered example
%% use: \begin{example}\extab\begin{tabular ...
%\newcommand{\extab}[2][-0.69\baselineskip]{ 
%   \parbox[t]{.9\textwidth}{
%     \setlength{\tabcolsep}{1.3pt} % use small space between columns
%     \vspace{#1}
%     #2
%    }
%}

% command to put ref in parentheses
\DeclareMathOperator*{\pinf}{\vphantom{p}inf}
\DeclareMathOperator*{\psup}{\vphantom{p}sup}
\renewcommand{\inf}{\pinf}
\renewcommand{\sup}{\psup}
%user defined commands
%\newcommand*\Mirr[1]{\textsc{Mirr} (#1)}
%\newcommand*\Wd[0]{\textit{W}_2}
%\newcommand*\dd[2]{\frac{\partial #1}{\partial #2}}
%\newcommand*\x[0]{\textbf{x}}
%\newcommand*\stein[1]{\mathcal{A}_{#1}}
%\newcommand*\w[0]{\textbf{w}}
%\newcommand*\at[2]{\left.#1\right|_{#2}}
%\newcommand*\ps[0]{p^*}
%\newcommand*\del[0]{\partial}
%\newcommand*\R[0]{\mathbb{R}}
%\newcommand*\Z[0]{\mathbb{Z}}

%NewSymbols








